Tail-GAN: Learning to Simulate Tail Risk Scenarios

The estimation of loss distributions for dynamic portfolios requires the simulation of scenarios representing realistic joint dynamics of their components. We propose a novel data-driven approach for simulating realistic, high-dimensional multi-asset scenarios, focusing on accurately representing tail risk for a class of static and dynamic trading strategies. We exploit the joint elicitability property of Value-at-Risk (VaR) and Expected Shortfall (ES) to design a Generative Adversarial Network (GAN) that learns to simulate price scenarios preserving these tail risk features. We demonstrate the performance of our algorithm on synthetic and market data sets through detailed numerical experiments. In contrast to previously proposed data-driven scenario generators, our proposed method correctly captures tail risk for a broad class of trading strategies and demonstrates strong generalization capabilities. In addition, combining our method with principal component analysis of the input data enhances its scalability to large-dimensional multi-asset time series, setting our framework apart from the univariate settings commonly considered in the literature.

==> results/Notation.tex <==
\begin{tabular}{ll}  
\hline
Symbol & Description \\\hline
$X \sim \mu$ & Random variable with distribution $\mu$\\
$\alpha$ & A specific quantile \\
$\mbox{VaR}_{\alpha}(\mu)$ & Value at Risk of distribution $\mu$ at $\alpha$ level \\
$\mbox{ES}_{\alpha}(\mu)$ & Expected Shortfall of distribution $\mu$ at $\alpha$ level \\
$S_{\alpha}(v,e,x)$ & Score \\
$H_1, H_2$ & Component functions in Score function \\
$M$ & Number of assets \\
$T$ & Periods \\
$\Delta$ & Duration of intervals \\
{{$\pmb{p} = \{(p_{m,t})_{t=1}^{T}\}_{m=1}^M$}} & Random matrix of price \\
$\pmb{p}_1, \cdots, \pmb{p}_N$ & $N$ IID samples of $\pmb{p}$ \\
$\mathbb{P}_r$ & Theoretical distribution of $\pmb{p}$ \\
$\mathbb{P}_r^{(n)}$ & Empirical distribution of $\mathbb{P}_r$ with $n$ samples\\
% $\hat{\mathbb{P}}^{N}_r$ & Empirical distribution of $\pmb{p}$ \\
$N_z$ & Dimension of noise \\
$L$ & Number of layers \\
$n_l$ & Width of the $l$-th layer \\
{{$\pmb{z}$}} & Input of the generator \\
$\pmb{W} = (\pmb{W}_l)_{l=1}^{L}, \pmb{b}=(\pmb{b}_l)_{l=1}^{L}$ & Parameters in the NN \\
$\sigma(\cdot)$ & Activation function \\
$G$ & Generator \\
$\mathcal{G}_{NN}$ & Class of generators \\
$\gamma$ & Parameters of Generator $G_{\gamma}(\cdot)$ (or $G(\cdot; \gamma)$)\\ %\hline
$\mathbb{P}_{G}$ & Theoretical distribution of price series generated by $G$ \\
$\mathbb{P}_{G}^{(n)}$ & Empirical distribution of $\mathbb{P}_{G}$ with $n$ samples\\
$K$ & Number of trading strategies \\
$\pmb{w} = (w_i)_{i=1}^{M}$ & Shares of $M$ assets in a static portfolio or dynamic strategy \\
$p_t(\pmb{w})$ & Market price of a combination $\pmb{w}$ \\
$A_t$ & Moving average estimator \\
$s_t(\pmb{w})$ & Trading signals \\
$s_U, s_L$ & Threshold to buy or short \\
$\overline{p}_t(\pmb{w},d)$ & Moving average price of the portfolio \\
$d_1, d_2$ & Durations of moving average estimator\\
$c$ & Cash budget \\ 
$\Pi^k$ & Strategy $k$ \\
{{$x^k = \Pi^{k}(\pmb{p})$}}& Final PnL of $\Pi^k$ at terminal time $T$\\
$\Pi^k\#\,\mathbb{P}_{r}$ & Theoretical distribution of $\Pi^{k}(\pmb{p})$ \\
$\Pi^k\#\,\mathbb{P}_{r}^{(n)}$ & Empirical distribution of $\Pi^k\#\,\mathbb{P}_{r}$ with $n$ samples \\
% $\mathbb{P}^{k}_{\text{PnL}, r}$ & Theoretical distribution of $\Pi^{k}(\pmb{p})$ \\
$\Pi^k\#\,\mathbb{P}_{G}$ & Theoretical distribution of $\Pi^{k}(G(\pmb{z}; \gamma))$  \\
$\Pi^k\#\,\mathbb{P}_{G}^{(n)}$ & Empirical distribution of $\Pi^k\#\,\mathbb{P}_{G}$ with $n$ samples \\
% $\mathbb{P}^{k}_{\text{PnL}, G} $ & Theoretical  distribution of $\Pi^{k}(G(\pmb{z}; \gamma))$ \\
$\pmb{\Pi} := (\Pi^1,\cdots,\Pi^K)$ & Mapping of all strategies \\%\hdashline
% $f_{\alpha}$ & Mapping $\alpha$-quantile VaR and ES values of distributions \\%\hline
$N_{B}$ & Number of PnL samples \\
{{$\{x^{k}_{i}\}_{i=1}^{N_{B}}$}} & PnL samples of strategy $k$\\
$\pmb{x}^{k} = (x^{k}_{i})_{i=1}^{N_{B}}$ & Vector of PnLs computed according to strategy $k$\\
$B(\pmb{x}^{k})$ & Absolute pairwise differences of the elements of $\pmb{x}^{k}$ \\
{{$\Gamma(\pmb{x}^{k})$}} & Permutation matrix of $\pmb{x}^{k}$ \\
$\mathcal{D}_{NN}$ & Class of discriminators \\
$\delta$ & Parameters of the discriminator $D_{\delta}(\cdot)$ (or $D(\cdot; \delta)$) \\\hline
\label{tab:notation}
\end{tabular}

==> results/Syn_VaRES_RE.tex <==
\begin{tabular}{l|ccccc}

            & SE(1000)   & HSM & {\TGAN-Raw} & {\TGAN-Static} & {\TGAN} \\\hline
Out-Of-Sample Error (\%)    &  3.0 & 3.4  & 83.3 & 86.7 & 4.6  \\
          &  (2.2) & (2.6) & (3.0) & (2.5) & (1.6) \\\hline
\end{tabular}

==> results/VaRES.tex <==
\begin{tabular}{l|c|c|c}
                                  & Epochs & In-Sample Error  & Out-Of-Sample Error\\\hline
single-asset portfolio            & 1130       & 0.151  & 0.172     \\
multi-asset portfolio             & 1840       & 0.080 & 0.074    \\
static portfolio+dynamic strategy & 1780       & 0.063 & 0.061    \\
\end{tabular}

==> results/algo.tex <==
\begin{algorithm}[H]
  \caption{{\TGAN}.}\label{alg:algorithm1}
  \hspace*{\algorithmicindent} \ \\
  \textbf{Input:}\\
  % Statex 
  \bb Price scenarios $\mathbf{p}_1,\dots,\mathbf{p}_{N_{}}\in\mathbb{R}^{M\times T}$. \\
  \bb Description of trading strategies: $\mathbf{\Pi}=(\Pi^1,\dots,\Pi^K) :\mathbb{R}^{M\times T}\to \mathbb{R}^K$.\\
  \bb Hyperparameters: learning rate $l_D$ for  discriminator  and $l_G$ for generator; number of training epochs; batch size $N_B$; dual parameter $\lambda$. 
   % \Statex 
\medskip 
  \begin{algorithmic}[1]
    %\Require
    %{\bf Inputs}\\
    %  \Statex Strategies $\mathbf{\Pi} := (\Pi^1,\ldots,\Pi^K)$, learning rate for the discriminator $l_D$ and the generator $l_G$, the number of training epoches and the batch size $N_B$.
    % \Statex
    \For{number of epochs} %\Comment{This line's number should be 1}
        \For{$j = 1 \to \floor{N/N_B}$}
            \State Generate  $N_B$ IID noise samples $\{\mathbf{z}_i, i\in[N_B]\}\sim \mathbb{P}_{\mathbf{z}}$.
            \State Sample a batch $\mathcal{B}_j \subset \{1,\dots,N\}$ of size  $N_B$ from the input data $\{\mathbf{p}_i, i =1, \dots, N\}$.
            \State Compute the loss of the discriminator on the batch $\mathcal{B}_j$
            \begin{equation} 
            \begin{aligned}
                \mathcal{L}_D(\mathbf{\delta}) = \frac{1}{K\,N_B}\,\, \sum_{k=1}^K \sum_{n\in \mathcal{B}_j}  
                &\Big[S_{\alpha}\big(D_{{\mathbf{\delta}}}(\Pi^k(G_{{\mathbf{\gamma}}}({\mathbf{z}_{i}})),i\in [N_B]), \Pi^k(\mathbf{p}_n)\big)\nonumber\\
                &-\lambda S_{\alpha}\big(D_{{\mathbf{\delta}}}(\Pi^k(\mathbf{p}_i), i \in \mathcal{B}_j), \Pi^k(\mathbf{p}_n)\big)\Big]. \nonumber
            \end{aligned}
            \end{equation}
            \State Update the discriminator 
            \begin{equation}
            \mathbf{\delta} \gets \mathbf{\delta} + l_D \nabla\mathcal{L}_D(\mathbf{\delta}). \nonumber
            \end{equation}
            \State Generate  $N_B$ IID noise samples $\{\tilde{\mathbf{z}}_i, i\in[N_B]\}\sim \mathbb{P}_{\mathbf{z}}$.
            \State Compute the loss of the generator
            \begin{equation}
            \begin{aligned}
                \mathcal{L}_G(\mathbf{\gamma})= \frac{1}{K\,N_B}\,\, \sum_{k=1}^K \sum_{n \in \mathcal{B}_j} S_{\alpha}\big(D_{{\delta}}(\Pi^k(G_{{\mathbf{\gamma}}}({\tilde{\mathbf{z}}_{i}})),i\in[N_B]), \Pi^k(\mathbf{p}_n)\big).
                \nonumber
            \end{aligned}
            \end{equation}  
            \State Update the generator 
            \begin{equation}
                \mathbf{\gamma} \gets \mathbf{\gamma} - l_G \nabla\mathcal{L}_G(\mathbf{\gamma}).   \nonumber  
            \end{equation}
        \EndFor
    \EndFor \\   $\mathbf{\gamma}^*= \mathbf{\gamma},\qquad \mathbf{\delta}^*=\mathbf{\delta}$.
   % \Statex
 \end{algorithmic}
 
 %\smallskip 
 \noindent \hspace*{\algorithmicindent} \ \\ \textbf{Outputs:}\\ 
 \bb  $\mathbf{\delta}^*$: trained discriminator weights; \quad  $\mathbf{\gamma}^*$: trained generator weights.\\
\bb  Simulated scenarios: $ G_{\mathbf{\gamma}^*}(\mathbf{z}_i)$ where $ \mathbf{z}_i\sim \mathbb{P}_{\mathbf{z}}$ IID.

\end{algorithm}

==> results/tmp_syn_VaRES.tex <==
\begin{tabular}{l|cccc}
                                              & 3 Stocks     & 3 Stocks + 3 Portfolios & 3 Stocks + 6 Portfolios & 3 Stocks + 9 Portfolios \\\hline
\# of IS Portfolios                           & 3            & 6                       & 9                       & 12                      \\
IS Relative Error                             & 0.103        & 0.057    & 0.107    & 0.055                   \\\hline
\# of IS Raw Stocks                           & 3            & 3                       & 3                       & 3                       \\
Relative Error of IS Raw Stocks               & 0.103        & 0.058    & 0.114    & 0.059                   \\\hdashline
\# of IS Static Portfolios                    & 0            & 3                       & 6                       & 9                       \\
{Relative Error of IS Static Portfolios} &  &  0.056    & 0.104    & 0.054                   \\\hline
\\
\\\hline
\# of OOS Portfolios                          & 16           & 16                      & 16                      & 16                      \\
OOS Relative Error                            & 0.133        & 0.092    & 0.105    & 0.071                    \\\hline
\# of OOS Static Portfolios                   & 10           & 10                      & 10                      & 10                      \\
Relative Error of OOS Static Portfolios       & 0.132        & 0.089    & 0.086    & 0.044                   \\\hdashline
\# of OOS Dynamic Portfolios                  & 6            & 6                       & 6                       & 6                       \\
Relative Error of OOS Dynamic Portfolios      & 0.136        & 0.097    & 0.137    & 0.118                  \\\hline
\end{tabular}

